Keyword-driven Retrieval-Augmented Large Language Models for Cold-start User Recommendations

Recent advancements in Large Language Models (LLMs) have shown significant potential in enhancing recommender systems. However, addressing the cold-start recommendation problem, where users lack historical data, remains a considerable challenge. In this paper, we introduce KALM4Rec (Keyword-driven Retrieval-Augmented Large Language Models for Cold-start User Recommendations), a novel framework specifically designed to tackle this problem by requiring only a few input keywords from users in a practical scenario of cold-start user restaurant recommendations. KALM4Rec operates in two main stages: candidates retrieval and LLM-based candidates re-ranking. In the first stage, keyword-driven retrieval models are used to identify potential candidates, addressing LLMs' limitations in processing extensive tokens and reducing the risk of generating misleading information. In the second stage, we employ LLMs with various prompting strategies, including zero-shot and few-shot techniques, to re-rank these candidates by integrating multiple examples directly into the LLM prompts. Our evaluation, using a Yelp restaurant dataset with user reviews from three English-speaking cities, shows that our proposed framework significantly improves recommendation quality. Specifically, the integration of in-context instructions with LLMs for re-ranking markedly enhances the performance of the cold-start user recommender system.

==> table/LLMs_compare.tex <==
\resizebox{1\columnwidth}{!}{%
{\setlength\doublerulesep{0.7pt}
\begin{tabular}{c|c|rrrrrrrr}
\toprule[1pt]\midrule[0.3pt]
\multicolumn{1}{c|}{Dataset}  & Methods & \multicolumn{1}{c}{P@1}   & \multicolumn{1}{c}{R@1}  & \multicolumn{1}{c}{P@3}   & \multicolumn{1}{c}{R@3}   & \multicolumn{1}{c}{N@3}   & \multicolumn{1}{c}{P@5} & \multicolumn{1}{c}{R@5} & \multicolumn{1}{c}{N@5} \\ \hline
\multirow{4}{*}{Yelp-Edinburgh} 
                           & CBR     & 29.15                     & 5.05                     & 19.13                     & 10.23                     & 32.81                     & 15.07                   & 13.19                   & 32.87                   \\
                           & CBR-LLM & \textbf{50.24}            & \textbf{10.16}           & \textbf{26.86}            & \textbf{14.17}            & \textbf{44.39}            & \textbf{18.92}          & \textbf{16.38}          & \textbf{40.34}          \\ \cline{2-10} 
                           & MPG     & 54.71                     & 10.91                    & 38.12                     & 20.55                     & 58.49                     & 30.40                   & 26.07                   & 55.86                   \\
                           & MPG-LLM & \textbf{61.69}            & \textbf{11.54}           & \textbf{42.95}            & \textbf{21.36}            & \textbf{62.19}            & \textbf{31.31}          & \textbf{26.77}          & \textbf{56.63}          \\ \hline
\multirow{4}{*}{Yelp-Singapore} & CBR     & 17.76                     & 3.98                     & 12.52                     & 8.10                      & 23.13                     & 10.56                   & 10.53                   & 23.91                   \\
                           & CBR-LLM & \textbf{29.44}            & \textbf{5.97}            & \textbf{17.93}            & \textbf{10.63}            & \textbf{32.82}            & \textbf{13.30}          & \textbf{13.11}          & \textbf{29.72}          \\ \cline{2-10} 
                           
                           & MPG     & 41.12                     & 8.19                     & 27.41                     & 15.55                     & 48.11                     & 22.34                   & 20.43         & 46.76          \\
                           & MPG-LLM & \textbf{51.78}            & \textbf{9.77}            & \textbf{31.13}            & \textbf{16.38}            & \textbf{51.05}            & \textbf{23.05}          & \textbf{23.05}          & \textbf{49.76}                   \\ \hline
\multirow{4}{*}{Yelp-London}    & CBR     & 26.06                     & 5.04                     & 17.45                     & 9.59                      & 31.46                     & 14.52                   & 13.09                   & 32.87                   \\
                           & CBR-LLM & \textbf{38.30}            & \textbf{7.75}            & \textbf{22.66}            & \textbf{12.94}            & \textbf{39.30}            & \textbf{17.31}          & \textbf{16.06}          & \textbf{39.34}        \\ \cline{2-10} 
                           & MPG     & \multicolumn{1}{c}{47.76} & \multicolumn{1}{c}{9.60} & \multicolumn{1}{c}{34.34} & \multicolumn{1}{c}{19.47} & \multicolumn{1}{c}{52.46} & 27.68                   & 25.17                   & 52.26                   \\
                           & MPG-LLM & \textbf{58.06}            & \textbf{11.77}           & \textbf{37.09}            & \textbf{20.67}            & \textbf{56.85}            & \textbf{29.18}          & \textbf{26.24}                   & \textbf{54.30}          \\ 
                           \hline
\multirow{4}{*}{TripAdvisor}    & CBR     & 21.38 & 3.35 & 15.30 & 7.16 & 28.92 & 12.99 & 10.00 & 31.23                   \\
                           & CBR-LLM & \textbf{36.27 }            & \textbf{5.79}            & \textbf{20.05}            & \textbf{9.42}            & \textbf{36.69}            & \textbf{14.84}          & \textbf{11.49}          & \textbf{11.49}        \\ \cline{2-10} 
                           & MPG     & \multicolumn{1}{c}{54.60} & {8.73} & {41.92} & {19.72} & {61.36} & {33.52} &
                            \textbf{25.98} &
                        {58.99}                    \\
                           & MPG-LLM & \textbf{59.43}            & \textbf{9.54}           & \textbf{42.15}            & \textbf{19.87}            & \textbf{62.36}            & \textbf{33.58}          & \textbf{25.98}                   & \textbf{59.65}          \\                            
                           \midrule[0.3pt] \bottomrule[1pt]
\end{tabular}
}%
}





% \resizebox{1.5\columnwidth}{!}{%
% {\setlength\doublerulesep{0.7pt}
% \begin{tabular}{c|c|rrrrrrrr}
% \toprule[1pt]\midrule[0.3pt]
% \multicolumn{1}{l|}{City}  & Methods & \multicolumn{1}{c}{P@1}   & \multicolumn{1}{c}{R@1}  & \multicolumn{1}{c}{P@3}   & \multicolumn{1}{c}{R@3}   & \multicolumn{1}{c}{N@3}   & \multicolumn{1}{c}{P@5} & \multicolumn{1}{c}{R@5} & \multicolumn{1}{c}{N@5} \\ \hline
% \multirow{4}{*}{Edinburgh} & MPG     & 54.71                     & 10.91                    & 38.12                     & 20.55                     & 58.49                     & 30.40                   & 26.07                   & 55.86                   \\
%                            & MPG-LLM & \textbf{61.69}            & \textbf{11.54}           & \textbf{42.95}            & \textbf{21.36}            & \textbf{62.19}            & \textbf{31.31}          & \textbf{26.77}          & \textbf{56.63}          \\ \cline{2-10} 
%                            & CBR     & 29.15                     & 5.05                     & 19.13                     & 10.23                     & 32.81                     & 15.07                   & 13.19                   & 32.87                   \\
%                            & CBR-LLM & \textbf{50.24}            & \textbf{10.16}           & \textbf{26.86}            & \textbf{14.17}            & \textbf{44.39}            & \textbf{18.92}          & \textbf{16.38}          & \textbf{40.34}          \\ \hline
% \multirow{4}{*}{Singapore} & MPG     & 41.12                     & 8.19                     & 27.41                     & 15.55                     & 48.11                     & 22.34                   & \textbf{20.43}          & \textbf{49.76}          \\
%                            & MPG-LLM & \textbf{51.78}            & \textbf{9.77}            & \textbf{31.13}            & \textbf{16.38}            & \textbf{51.05}            & \textbf{23.05}          & \textbf{23.05}          & 46.76                   \\ \cline{2-10} 
%                            & CBR     & 17.76                     & 3.98                     & 12.52                     & 8.10                      & 23.13                     & 10.56                   & 10.53                   & 23.91                   \\
%                            & CBR-LLM & \textbf{29.44}            & \textbf{5.97}            & \textbf{17.93}            & \textbf{10.63}            & \textbf{32.82}            & \textbf{13.30}          & \textbf{13.11}          & \textbf{29.72}          \\ \hline
% \multirow{4}{*}{London}    & MPG     & \multicolumn{1}{c}{47.76} & \multicolumn{1}{c}{9.60} & \multicolumn{1}{c}{34.34} & \multicolumn{1}{c}{19.47} & \multicolumn{1}{c}{52.46} & 27.68                   & 25.17                   & 52.26                   \\
%                            & MPG-LLM & \textbf{55.15}            & \textbf{11.19}           & \textbf{36.48}            & \textbf{20.48}            & \textbf{55.40}            & \textbf{28.53}          & 26.89                   & \textbf{54.03}          \\ \cline{2-10} 
%                            & CBR     & 26.06                     & 5.04                     & 17.45                     & 9.59                      & 31.46                     & 14.52                   & 13.09                   & 32.87                   \\
%                            & CBR-LLM & \textbf{38.30}            & \textbf{7.75}            & \textbf{22.66}            & \textbf{12.94}            & \textbf{39.30}            & \textbf{17.31}          & \textbf{16.06}          & \textbf{39.34}        \\ \midrule[0.3pt] \bottomrule[1pt]
% \end{tabular}
% }%
% }

==> table/kw_extractor.tex <==
\resizebox{1.0\columnwidth}{!}{%
{\setlength\doublerulesep{0.7pt}
\begin{tabular}{l|llllllll}
\toprule[1pt]\midrule[0.3pt]
\multicolumn{1}{c|}{}                          & \multicolumn{6}{c}{Keyword Extractors}                                                     \\ \cline{2-9} 
\multicolumn{1}{c|}{}                          & \multicolumn{2}{c}{spaCy}            & \multicolumn{2}{c}{Rake} & \multicolumn{2}{c}{Yake}  & \multicolumn{2}{c}{NLTK} \\ \cline{2-9} 
\multicolumn{1}{c|}{\multirow{-3}{*}{Dataset}} & P@20  & R@20                         & P@20        & R@20       & P@20        & R@20 & P@20        & R@20      \\ \hline
Edinburgh                                      & \textbf{14.42} & {\color[HTML]{242424} \textbf{40.44}} & {\ul 13.5}    & 36.89    & 13.21       & {\ul 37.6} & 9.14 & 30.87   \\
Singapore                                      & \textbf{10.38} & {\color[HTML]{242424} {\ul 34.86}}    & 9.47          & 32.82    & {\ul 10.36} & \textbf{35.91} & 8.12	& 27.56 \\
London                                         & \textbf{12.73} & \textbf{41.44}                        & 11.58         & 37.93    & {\ul 12.07} & {\ul 39.68}   & 9.29 &	32.19 \\
TripAdvisor                                    & \textbf{14.54} & \textbf{43.74}                        & 13.41         & 40.18    & { 13.74} & { 41.28} & {\ul 14.17} & {\ul 43.16}    \\
\midrule[0.3pt] \bottomrule[1pt]
\end{tabular}
}%
}

==> table/llm_comparison_method_prompting.tex <==
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllllll}

\multicolumn{1}{l|}{Method}   & \multicolumn{1}{l}{P@1}    & \multicolumn{1}{l}{R@1}    & \multicolumn{1}{l}{P@3}    & \multicolumn{1}{l}{R@3}    & \multicolumn{1}{l}{P@5}    & R@5    \\ \hline
\multicolumn{7}{c}{Edinburgh}                                                                                                                                                               \\ \hline
\multicolumn{1}{l|}{Baseline} & \multicolumn{1}{l|}{0.5471} & \multicolumn{1}{l|}{0.1091} & \multicolumn{1}{l|}{0.3812} & \multicolumn{1}{l|}{0.2055} & \multicolumn{1}{l|}{0.3040} & 0.2607 \\ 
\multicolumn{1}{l|}{zeroshot} & \multicolumn{1}{l|}{0.5785} & \multicolumn{1}{l|}{0.1177} & \multicolumn{1}{l|}{0.3842} & \multicolumn{1}{l|}{0.2089} & \multicolumn{1}{l|}{0.2960} & 0.2504 \\ 
\multicolumn{1}{l|}{1 shot}   & \multicolumn{1}{l|}{0.5919} & \multicolumn{1}{l|}{0.1222} & \multicolumn{1}{l|}{0.3946} & \multicolumn{1}{l|}{0.2147} & \multicolumn{1}{l|}{0.3031} & 0.2586 \\ 
\multicolumn{1}{l|}{2 shot}   & \multicolumn{1}{l|}{0.5874} & \multicolumn{1}{l|}{0.1214} & \multicolumn{1}{l|}{0.3871} & \multicolumn{1}{l|}{0.2165} & \multicolumn{1}{l|}{0.2861} & 0.2507 \\ 
\multicolumn{1}{l|}{3 shot}   & \multicolumn{1}{l|}{0.5964} & \multicolumn{1}{l|}{0.1217} & \multicolumn{1}{l|}{0.3797} & \multicolumn{1}{l|}{0.2125} & \multicolumn{1}{l|}{0.2861} & 0.2506 \\ \hline
\multicolumn{7}{c}{London}                                                                                                                                                                  \\ \hline
\multicolumn{1}{l|}{Baseline} & \multicolumn{1}{l|}{0.4485} & \multicolumn{1}{l|}{0.0893} & \multicolumn{1}{l|}{0.3188} & \multicolumn{1}{l|}{0.1837} & \multicolumn{1}{l|}{0.2509} & 0.2331 \\ 
\multicolumn{1}{l|}{zeroshot} & \multicolumn{1}{l|}{0.5127} & \multicolumn{1}{l|}{0.1025} & \multicolumn{1}{l|}{0.3418} & \multicolumn{1}{l|}{0.1957} & \multicolumn{1}{l|}{0.2658} & 0.2400 \\ 
\multicolumn{1}{l|}{1 shot}   & \multicolumn{1}{l|}{0.5018} & \multicolumn{1}{l|}{0.1030} & \multicolumn{1}{l|}{0.3402} & \multicolumn{1}{l|}{0.1943} & \multicolumn{1}{l|}{0.2630} & 0.2391 \\ 
\multicolumn{1}{l|}{2 shot}   & \multicolumn{1}{l|}{0.5067} & \multicolumn{1}{l|}{0.1016} & \multicolumn{1}{l|}{0.3370} & \multicolumn{1}{l|}{0.1907} & \multicolumn{1}{l|}{0.2628} & 0.2396 \\ 
\multicolumn{1}{l|}{3 shot}   & \multicolumn{1}{l|}{0.5321} & \multicolumn{1}{l|}{0.1087} & \multicolumn{1}{l|}{0.3463} & \multicolumn{1}{l|}{0.1965} & \multicolumn{1}{l|}{0.2635} & 0.2399 \\ \hline
\end{tabular}%
}

==> table/llm_fewshot.tex <==
\resizebox{0.3\textwidth}{!}{%
\begin{tabular}{l|l|ll}
\toprule[1pt]\midrule[0.3pt]
City  & \multicolumn{1}{c|}{MPG} & \multicolumn{1}{c}{Few-shot}  \\ \hline
Edinburgh  & 0.547 & 0.617 ($\uparrow$\textit{12.8}\%)  \\
Singapore  & 0.411 & 0.548 ($\uparrow$\textit{33.3}\%)  \\
London     & 0.448 & 0.535 ($\uparrow$\textit{19.4}\%)  \\
Charlotte  & 0.538 & 0.572 ($\uparrow$\textit{6.3}\%)   \\
Lasvegas   & 0.576 & 0.583 ($\uparrow$\textit{1.2}\%)   \\
Pittsburgh & 0.637 & 0.746 ($\uparrow$\textit{17.11}\%)  \\
Phoenix    & 0.642 & 0.731 ($\uparrow$\textit{13.86}\%)  \\ \midrule[0.3pt] \bottomrule[1pt]
\end{tabular}%
}

==> table/llms_all.tex <==
\resizebox{0.9\columnwidth}{!}{%
{\setlength\doublerulesep{0.7pt}
\begin{tabular}{l|c|ccccc}
\toprule[1pt]\midrule[0.3pt]
City Name                  & Model                          & \multicolumn{1}{c}{P@1} & \multicolumn{1}{c}{R@1} & \multicolumn{1}{c}{P@3} & \multicolumn{1}{c}{R@3} & \multicolumn{1}{c}{N@3} \\ \hline
\multirow{5}{*}{Edinburgh} & MPG                            & 54.71                   & 10.91                   & 38.12                   & 20.55                   & 58.49                   \\ \cline{2-7}
                           & Gemini                         & \textbf{61.69}          & {\ul 11.54}             & \textbf{42.95}          & \textbf{21.36}          & \textbf{62.19}          \\
                           & GPT-3.5                        & 56.05                   & 11.21                   & {\ul 38.86}             & {\ul 21.26}             & 58.72                   \\
                           & Mistral 8B                             & {\ul 58.30}             & \textbf{11.85}          & 37.82                   & 20.87                   & {\ul 60.16}             \\
                           & \multicolumn{1}{l|}{Llama3 8B} & 56.50                   & 11.27                   & 36.62                   & 18.91                   & 56.42                   \\ \hline
\multirow{5}{*}{Singapore} & MPG                            & 41.12                   & 8.19                    & 27.41                   & 15.55                   & 48.11                   \\\cline{2-7}
                           & Gemini                         & \textbf{51.78}          & \textbf{9.77}           & \textbf{31.13}          & \textbf{16.38}          & {\ul 51.05}          \\
                           & GPT-3.5                        & 48.73                   & 8.85                    & {\ul 30.29}             & 16.22                   & \textbf{51.86}             \\
                           & Mistral 8B                             & {\ul 49.75}                   & {\ul 9.67}           & {\ul 30.29}             & {\ul 16.27}             & 50.02                   \\
                           & \multicolumn{1}{l|}{Llama3 8B} & 45.18                   & 8.71                    & 29.10                   & 14.99                   & 49.27                   \\ \hline
\multirow{5}{*}{London}    & MPG                            & 47.76                   & 9.60                    & 34.34                   & 19.47                   & 52.46                   \\\cline{2-7}
                           & Gemini                         & \textbf{58.06}            & \textbf{11.77}           & \textbf{37.09}            & \textbf{20.67}            & \textbf{56.85}         \\
                           & GPT-3.5                        & 52.97                   & {\ul 10.81}             & 34.00                   & {\ul 19.38}             & 53.96                   \\
                           & Mistral 8B                             & {\ul 53.82}             & 10.79                   & 33.74                   & 18.87                   & {\ul 54.21}             \\
                           & \multicolumn{1}{l|}{Llama3 8B} & 51.64                   & 10.39                   & {\ul 34.08}             & 18.83                   & 53.49             \\ \midrule[0.3pt] \bottomrule[1pt]
\end{tabular}
\vspace{-0.2in}
}%
}

% \resizebox{1\columnwidth}{!}{%
% {\setlength\doublerulesep{0.7pt}
% \begin{tabular}{l|c|ccccc}
% \toprule[1pt]\midrule[0.3pt]
% City Name                  & Model                          & \multicolumn{1}{c}{p@1} & \multicolumn{1}{c}{r@1} & \multicolumn{1}{c}{p@3} & \multicolumn{1}{c}{r@3} & \multicolumn{1}{c}{n@3} \\ \hline
% \multirow{5}{*}{Edinburgh} & MPG                            & 54.71                   & 10.91                   & 38.12                   & 20.55                   & 58.49                   \\
%                            & Gemini                         & \textbf{61.69}          & {\ul 11.54}             & \textbf{42.95}          & \textbf{21.36}          & \textbf{62.19}          \\
%                            & ChatGPT                        & 56.05                   & 11.21                   & {\ul 38.86}             & {\ul 21.26}             & 58.72                   \\
%                            & 8B                             & {\ul 58.30}             & \textbf{11.85}          & 37.82                   & 20.87                   & {\ul 60.16}             \\
%                            & \multicolumn{1}{l|}{Llama3 8B} & 56.50                   & 11.27                   & 36.62                   & 18.91                   & 56.42                   \\ \hline
% \multirow{5}{*}{Singapore} & MPG                            & 41.12                   & 8.19                    & 27.41                   & 15.55                   & 48.11                   \\
%                            & Gemini                         & \textbf{51.78}          & \textbf{9.77}           & \textbf{31.13}          & \textbf{16.38}          & \textbf{51.05}          \\
%                            & ChatGPT                        & 48.73                   & 8.85                    & {\ul 30.29}             & 16.22                   & {\ul 51.86}             \\
%                            & 8B                             & 49.75                   & \textbf{9.67}           & {\ul 30.29}             & {\ul 16.27}             & 50.02                   \\
%                            & \multicolumn{1}{l|}{Llama3 8B} & 45.18                   & 8.71                    & 29.10                   & 14.99                   & 49.27                   \\ \hline
% \multirow{5}{*}{London}    & MPG                            & 47.76                   & 9.60                    & 34.34                   & 19.47                   & 52.46                   \\
%                            & Gemini                         & \textbf{55.15}          & \textbf{11.19}          & \textbf{36.48}          & \textbf{20.48}          & \textbf{55.40}          \\
%                            & ChatGPT                        & 52.97                   & {\ul 10.81}             & 34.00                   & {\ul 19.38}             & 53.96                   \\
%                            & 8B                             & {\ul 53.82}             & 10.79                   & 33.74                   & 18.87                   & {\ul 54.21}             \\
%                            & \multicolumn{1}{l|}{Llama3 8B} & 51.64                   & 10.39                   & {\ul 34.08}             & 18.83                   & 53.49             \\ \midrule[0.3pt] \bottomrule[1pt]
% \end{tabular}
% }%
% }
